Linked visualisations via Galois dependencies

We present new language-based dynamic analysis techniques for linking visualisations and other structured outputs to data in a fine-grained way, allowing a user to interactively explore how data attributes map to visual or other output elements by selecting (focusing on) substructures of interest. This can help both programmers and end-users understand how data sources and complex outputs are related, which can be a challenge even for someone with expert knowledge of the problem domain. Our approach builds on bidirectional program slicing techiques based on Galois connections, which provide desirable round-tripping properties. Unlike the prior work in program slicing, our approach allows selections to be negated. In a setting with negation, the bidirectional analysis has a De Morgan dual, which can be used to link different outputs generated from the same input. This offers a principled language-based foundation for a popular interactive visualisation feature called brushing and linking where selections in one chart automatically select corresponding elements in another related chart. Although such view coordination features are valuable comprehension aids, they tend be to hard-coded into specific applications or libraries, or require programmer effort.

==> fig/core-language/slicing/join-elim.tex <==
\begin{figure}[H]
\flushleft\shadebox{$\sigma \join \sigma'$}
\begin{salign}
   \hole \join \sigma &= \sigma
   \\
   \sigma \join \hole &= \sigma
   \\
   (\elimVar{x}{\kappa}) \join (\elimVar{x}{\kappa'})
   &=
   \elimVar{x}{\kappa \join \kappa'}
   \\
   \elimBool{\kappa_1}{\kappa_2} \join \elimBool{\kappa_1'}{\kappa_2'}
   &=
   \elimBool{\kappa_1 \join \kappa_1'}{\kappa_2 \join \kappa_2'}
   \\
   \elimRec{\vec{x}}{\kappa} \join \elimRec{\vec{x}}{\kappa'}
   &=
   \elimRec{\vec{x}}{\kappa \join \kappa'}
   \\
   \elimList{\kappa}{\sigma} \join \elimList{\kappa'}{\sigma'}
   &=
   \elimList{\kappa \join \kappa'}{\sigma \join \sigma'}
\end{salign}
\caption{Join of compatible eliminators}
\label{fig:join-elim}
\end{figure}


==> fig/core-language/slicing/join-value.tex <==
\begin{figure}[H]
\flushleft\shadebox{$h \join h'$}
\begin{salign}
   \vec{\bind{x}{\sigma}} \join \vec{\bind{x}{\tau}}
   =
   \vec{\bind{x}{\sigma \join \tau}}
\end{salign}

\vspace{5pt}
\flushleft\shadebox{$v \join v'$}
\begin{salign}
   \hole \join v &= v
   \\
   v \join \hole &= v
   \\
   \annTrue{\alpha} \join \annTrue{\alpha'} &= \annTrue{\alpha \join \alpha'}
   \\
   \annFalse{\alpha} \join \annFalse{\alpha'} &= \annFalse{\alpha \join \alpha'}
   \\
   \annInt{n}{\alpha} \join \annInt{n}{\alpha'} &= \annInt{n}{\alpha \join \alpha'}
   \\
   \annRec{\vec{\bind{x}{u}}}{\alpha} \join \annRec{\vec{\bind{x}{v}}}{\alpha'} &=
   \annRec{\vec{\bind{x}{u \join v}}}{\alpha \join \alpha'}
   \\
   \annNil{\alpha} \join \annNil{\alpha} &= \annNil{\alpha \join \alpha'}
   \\
   (\annCons{u}{v}{\alpha}) \join (\annCons{u'}{v'}{\alpha'})
   &=
   \annCons{(u \join u')}{(v \join v')}{\alpha \join \alpha'}
   \\
   \annVecVal{\vec{v}}{\annInt{j}{\beta}}{\alpha}
   \join
   \annVecVal{\vec{u}}{\annInt{j}{\beta'}}{\alpha'}
   &=
   \annVecVal{\vec{v \join u}}
             {\annInt{j}{\beta \join \beta'}}{\alpha \join \alpha'}
   \\
   \exPrimOp{\phi}{\vec{v}} \join
   \exPrimOp{\phi}{\vec{u}}
   &=
   \exPrimOp{\phi}{\vec{v \join u}}
   \\
   \exClosure{\rho}{h}{\sigma} \join \exClosure{\rho'}{h'}{\sigma'}
   &=
   \exClosure{\rho \join \rho'}{h \join h'}{\sigma \join \sigma'}
\end{salign}
\caption{Join of compatible values}
\label{fig:join-value}
\end{figure}


==> fig/core-language/slicing/leq-elim-term.tex <==
\flushleft \shadebox{$h \leq h'$}
\begin{smathpar}
   \inferrule*[
   ]
   {
      \sigma_i \leq \tau_i
      \quad
      (\forall i \numleq \length{\vec{x}})
   }
   {
      \vec{\bind{x}{\sigma}}
      \leq
      \vec{\bind{x}{\tau}}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \sigma_i \leq \hole
      \quad
      (\forall i \numleq \length{x})
   }
   {
      \vec{\bind{x}{\sigma}} \leq \hole
   }
\end{smathpar}

\vspace{5pt}
\flushleft \shadebox{$e \leq e'$}
\begin{smathpar}
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \hole \leq e
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \alpha \leq \alpha'
   }
   {
      \annInt{n}{\alpha} \leq \annInt{n}{\alpha'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \annInt{n}{\bot} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \alpha \leq \alpha'
   }
   {
      \annTrue{\alpha} \leq \annTrue{\alpha'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \annTrue{\bot} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \alpha \leq \alpha'
   }
   {
      \annFalse{\alpha} \leq \annFalse{\alpha'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \annFalse{\bot} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \alpha \leq \alpha'
      \quad
      e_i \leq e'_i
      \quad
      (\forall i \numleq \length{\vec{x}})
   }
   {
      \annRec{\vec{\bind{x}{e}}}{\alpha} \leq \annRec{\vec{\bind{x}{e}}'}{\alpha'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      e_i \leq \hole
      \quad
      (\forall i \numleq \length{\vec{x}})
   }
   {
      \annRec{\vec{\bind{x}{e}}}{\bot} \leq \hole
   }
   %
   \and
   %
   \inferrule*
   {
      e \leq e'
   }
   {
      \exRecProj{e}{x} \leq \exRecProj{e'}{x}
   }
   %
   \and
   %
   \inferrule*
   {
      e \leq \hole
   }
   {
      \exRecProj{e}{x} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \alpha \leq \alpha'
   }
   {
      \annNil{\alpha} \leq \annNil{\alpha'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \annNil{\bot} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
      right={$\alpha \leq \alpha'$}
   ]
   {
      e_1 \leq e_1'
      \\
      e_2 \leq e_2'
   }
   {
      \annCons{e_1}{e_2}{\alpha} \leq \annCons{e_1'}{e_2'}{\alpha'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      e_1 \leq \hole
      \\
      e_2 \leq \hole
   }
   {
      \annCons{e_1}{e_2}{\bot} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \exVar{x} \leq \exVar{x}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \exVar{x} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \sigma \leq \sigma'
   }
   {
      \exLambda{\sigma} \leq \exLambda{\sigma}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \sigma \leq \hole
   }
   {
      \exLambda{\sigma} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      e_1 \leq e_1'
      \\
      e_2 \leq e_2'
   }
   {
      \exApp{e_1}{e_2} \leq \exApp{e_1}{e_2}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      e_1 \leq \hole
      \\
      e_2 \leq \hole
   }
   {
      \exApp{e_1}{e_2} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      e_1 \leq \hole
      \\
      e_2 \leq \hole
   }
   {
      \exLet{x}{e_1}{e_2} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      e \leq e'
      \\
      h \leq h'
   }
   {
      \exLetRecMutual{h}{e} \leq \exLetRecMutual{h'}{e'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      e \leq \hole
      \\
      h \leq \hole
   }
   {
      \exLetRecMutual{h}{e} \leq \hole
   }
\end{smathpar}

\vspace{5pt}
\flushleft \shadebox{$\sigma \leq \sigma'$}
\begin{smathpar}
   \inferrule*[
   ]
   {
      \strut
   }
   {
      \hole \leq \sigma
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \kappa \leq \kappa'
   }
   {
      \elimVar{x}{\kappa} \leq \elimVar{x}{\kappa'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \kappa \leq \hole
   }
   {
      \elimVar{x}{\kappa} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \kappa_1 \leq \kappa_1'
      \\
      \kappa_1 \leq \kappa_1'
   }
   {
      \elimBool{\kappa_1}{\kappa_2} \leq \elimBool{\kappa_1'}{\kappa_2'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \kappa_1 \leq \hole
      \\
      \kappa_1 \leq \hole
   }
   {
      \elimBool{\kappa_1}{\kappa_2} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \sigma \leq \sigma'
   }
   {
      \elimRec{\vec{x}}{\sigma} \leq \elimRec{\vec{x}}{\sigma'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \sigma \leq \hole
   }
   {
      \elimRec{\vec{x}}{\sigma} \leq \hole
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \kappa \leq \kappa'
      \\
      \sigma \leq \sigma'
   }
   {
      \elimList{\kappa}{\sigma} \leq \elimList{\kappa'}{\sigma'}
   }
   %
   \and
   %
   \inferrule*[
   ]
   {
      \kappa \leq \hole
      \\
      \sigma \leq \hole
   }
   {
      \elimList{\kappa}{\sigma} \leq \hole
   }
\end{smathpar}


==> fig/core-language/typing-value.tex <==
\begin{figure}[H]
\caption{Typing rules for environments and values}
\label{core-typing-value}
\end{figure}


==> sed-commands <==
s/>=/$\\numgeq$/g
s/<=/$\\numleq$/g
s/<-/$\\leftarrow$/g
s/->/$\\rightarrow$/g
s/\[|/\$\\langle$/g
s/|\]/$\\rangle$/g


==> tex-common/MnSymbol-asterisk.tex <==
% Bring in asterisk symbols from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\Mnthinstar}{\mathrel}{MnSyC}{134}
\DeclareMathSymbol{\Mnast}{\mathrel}{MnSyC}{135}


==> tex-common/MnSymbol-bowtie.tex <==
\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\let\bowtie\relax
\DeclareMathSymbol{\bowtie}{\mathrel}{MnSyC}{38}


==> tex-common/MnSymbol-cong.tex <==
% Bring in \cong from MnSymbol.

\DeclareFontFamily{U}{MnSymbolD}{}
\DeclareFontShape{U}{MnSymbolD}{m}{n}{
    <-6>  MnSymbolD5
   <6-7>  MnSymbolD6
   <7-8>  MnSymbolD7
   <8-9>  MnSymbolD8
   <9-10> MnSymbolD9
  <10-12> MnSymbolD10
  <12->   MnSymbolD12}{}
\DeclareFontShape{U}{MnSymbolD}{b}{n}{
    <-6>  MnSymbolD-Bold5
   <6-7>  MnSymbolD-Bold6
   <7-8>  MnSymbolD-Bold7
   <8-9>  MnSymbolD-Bold8
   <9-10> MnSymbolD-Bold9
  <10-12> MnSymbolD-Bold10
  <12->   MnSymbolD-Bold12}{}
\DeclareSymbolFont{MnSyD}{U}{MnSymbolD}{m}{n}

\DeclareMathSymbol{\Cong}{\mathrel}{MnSyD}{12}


==> tex-common/MnSymbol-inequalities.tex <==
\DeclareFontFamily{U}{MnSymbolD}{}
\DeclareFontShape{U}{MnSymbolD}{m}{n}{
    <-6>  MnSymbolD5
   <6-7>  MnSymbolD6
   <7-8>  MnSymbolD7
   <8-9>  MnSymbolD8
   <9-10> MnSymbolD9
  <10-12> MnSymbolD10
  <12->   MnSymbolD12}{}
\DeclareFontShape{U}{MnSymbolD}{b}{n}{
    <-6>  MnSymbolD-Bold5
   <6-7>  MnSymbolD-Bold6
   <7-8>  MnSymbolD-Bold7
   <8-9>  MnSymbolD-Bold8
   <9-10> MnSymbolD-Bold9
  <10-12> MnSymbolD-Bold10
  <12->   MnSymbolD-Bold12}{}
\DeclareSymbolFont{MnSyD}{U}{MnSymbolD}{m}{n}

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\sqcupdot}{\mathrel}{MnSyC}{68}
\DeclareMathSymbol{\sqcapdot}{\mathrel}{MnSyC}{69}
\DeclareMathSymbol{\eqslantgtr}{\mathrel}{MnSyC}{228}
\DeclareMathSymbol{\eqslantless}{\mathrel}{MnSyC}{227}

\DeclareMathSymbol{\less}{\mathrel}{MnSyD}{64}
\DeclareMathSymbol{\gtr}{\mathrel}{MnSyD}{65}
\DeclareMathSymbol{\leqslant}{\mathrel}{MnSyD}{68}
\DeclareMathSymbol{\geqslant}{\mathrel}{MnSyD}{69}
\DeclareMathSymbol{\sqlt}{\mathrel}{MnSyD}{88}
\DeclareMathSymbol{\sqgt}{\mathrel}{MnSyD}{89}
\DeclareMathSymbol{\sqleq}{\mathrel}{MnSyD}{90}
\DeclareMathSymbol{\sqgeq}{\mathrel}{MnSyD}{91}
\DeclareMathSymbol{\lessdot}{\mathrel}{MnSyD}{114}
\DeclareMathSymbol{\greaterdot}{\mathrel}{MnSyD}{115}
\DeclareMathSymbol{\leqslantdot}{\mathrel}{MnSyD}{118}
\DeclareMathSymbol{\geqslantdot}{\mathrel}{MnSyD}{119}
\DeclareMathSymbol{\leqslant}{\mathrel}{MnSyD}{68}
\DeclareMathSymbol{\geqslant}{\mathrel}{MnSyD}{69}
\DeclareMathSymbol{\nsqleq}{\mathrel}{MnSyD}{210}
\DeclareMathSymbol{\nsqgeq}{\mathrel}{MnSyD}{211}


==> tex-common/MnSymbol-medsquare.tex <==
% Bring in \medsquare from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\medsquare}{\mathord}{MnSyC}{106}


==> tex-common/MnSymbol-powerset.tex <==
% Bring in \powerset from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\MnSymbolpowerset}{\mathord}{MnSyC}{180}


==> tex-common/MnSymbol-triangles.tex <==
% Various triangles from MnSymbol. See http://tex.stackexchange.com/questions/36006.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\smalltriangleright}{\mathord}{MnSyC}{72}
\DeclareMathSymbol{\smalltriangleup}{\mathord}{MnSyC}{73}
\DeclareMathSymbol{\smalltriangleleft}{\mathord}{MnSyC}{74}
\DeclareMathSymbol{\smalltriangledown}{\mathord}{MnSyC}{75}
\DeclareMathSymbol{\filledtriangleright}{\mathord}{MnSyC}{76}
\DeclareMathSymbol{\filledtriangleup}{\mathord}{MnSyC}{77}
\DeclareMathSymbol{\filledtriangleleft}{\mathord}{MnSyC}{78}
\DeclareMathSymbol{\filledtriangledown}{\mathord}{MnSyC}{79}


==> tex-common/MnSymbol-twoheadarrows.tex <==
\DeclareFontFamily{U}{MnSymbolB}{}
\DeclareFontShape{U}{MnSymbolB}{m}{n}{
    <-6>  MnSymbolB5
   <6-7>  MnSymbolB6
   <7-8>  MnSymbolB7
   <8-9>  MnSymbolB8
   <9-10> MnSymbolB9
  <10-12> MnSymbolB10
  <12->   MnSymbolB12}{}
\DeclareFontShape{U}{MnSymbolB}{b}{n}{
    <-6>  MnSymbolB-Bold5
   <6-7>  MnSymbolB-Bold6
   <7-8>  MnSymbolB-Bold7
   <8-9>  MnSymbolB-Bold8
   <9-10> MnSymbolB-Bold9
  <10-12> MnSymbolB-Bold10
  <12->   MnSymbolB-Bold12}{}
\DeclareSymbolFont{MnSyB}{U}{MnSymbolB}{m}{n}

\DeclareFontFamily{U}{MnSymbolA}{}
\DeclareFontShape{U}{MnSymbolA}{m}{n}{
    <-6>  MnSymbolA5
   <6-7>  MnSymbolA6
   <7-8>  MnSymbolA7
   <8-9>  MnSymbolA8
   <9-10> MnSymbolA9
  <10-12> MnSymbolA10
  <12->   MnSymbolA12}{}
\DeclareFontShape{U}{MnSymbolA}{b}{n}{
    <-6>  MnSymbolA-Aold5
   <6-7>  MnSymbolA-Aold6
   <7-8>  MnSymbolA-Aold7
   <8-9>  MnSymbolA-Aold8
   <9-10> MnSymbolA-Aold9
  <10-12> MnSymbolA-Aold10
  <12->   MnSymbolA-Aold12}{}
\DeclareSymbolFont{MnSyA}{U}{MnSymbolA}{m}{n}

\let\twoheaddownarrow\relax
\DeclareMathSymbol{\twoheaddownarrow}{\mathrel}{MnSyA}{27}
\let\twoheaduparrow\relax
\DeclareMathSymbol{\twoheaduparrow}{\mathrel}{MnSyA}{25}

\let\ntwoheaddownarrow\relax
\DeclareMathSymbol{\ntwoheaddownarrow}{\mathrel}{MnSyB}{27}
\let\ntwoheaduparrow\relax
\DeclareMathSymbol{\ntwoheaduparrow}{\mathrel}{MnSyB}{25}


==> tex-common/MnSymbol-vdots.tex <==
% Bring in \medsquare from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\MnSymbolvdots}{\mathord}{MnSyC}{6}


==> tex-common/bigcdot.tex <==
% http://tex.stackexchange.com/questions/235118
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.7}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother


==> tex-common/curvetie.tex <==
% https://tex.stackexchange.com/questions/371292
% other solution based on halloweenmath, which is no longer in my TeX distribution...

\RequirePackage{pict2e}

\makeatletter
\DeclareRobustCommand{\curvetie}{\mathbin{\mathpalette\arc@bow@tie\relax}}
\newcommand{\arc@bow@tie}[2]{%
  \vcenter{\hbox{%
    \sbox\z@{$\m@th#1\otimes$}%
    \sbox\tw@{$\m@th\mkern1mu$}%
    \setlength{\unitlength}{\wd\z@}%
    \linethickness{.4\wd\tw@}%
    \begin{picture}(1,1)
    \polyline(0.7878,0.7878)(0.2122,0.2122)
    \polyline(0.2122,0.7878)(0.7878,0.2122)
    \put(0.5,0.5){\arc[-46,46]{0.4}}
    \put(0.5,0.5){\arc[134,226]{0.4}}
    \end{picture}%
  }}%
}
\makeatother


==> tex-common/line-shift.tex <==
% shift left, shift right line styles.

\usetikzlibrary{decorations}
\pgfdeclaredecoration{simple line}{initial}{
  \state{initial}[width=\pgfdecoratedpathlength-1sp]{\pgfmoveto{\pgfpointorigin}}
  \state{final}{\pgflineto{\pgfpointorigin}}
}
\tikzset{
   shift left/.style={decorate,decoration={simple line,raise=#1}},
   shift right/.style={decorate,decoration={simple line,raise=-1*#1}},
}


==> tex-common/mathabx-barharpoons.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathb10
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\leftbarharpoon}        {3}{mathb}{"DC}
\DeclareMathSymbol{\rightbarharpoon}       {3}{mathb}{"DD}
\DeclareMathSymbol{\barleftharpoon}        {3}{mathb}{"DE}
\DeclareMathSymbol{\barrightharpoon}       {3}{mathb}{"DF}


==> tex-common/mathabx-bigoslash.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\bigoslash}{1}{mathx}{"CD}


==> tex-common/mathabx-bigotimes.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\bigotimes}{1}{mathx}{"C2}


==> tex-common/mathabx-primes.tex <==
% Setup the matha font (from mathabx.sty) -- because mathabx.sty incompatible with
% amsmath package.
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * matha
      <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
      }{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}

% Define some characters from mathabx.dcl.
\DeclareMathSymbol{\twoPrime}{3}{matha}{"32}
\DeclareMathSymbol{\threePrime}{3}{matha}{"33}
\DeclareMathSymbol{\fourPrime}{3}{matha}{"34}


==> tex-common/mathabx-sqbullet.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathb10
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\sqbullet}{1}{mathb}{"0D}


==> tex-common/mathabx-wideparen.tex <==
% https://tex.stackexchange.com/questions/69323

%% code from mathabx.sty and mathabx.dcl
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}
\DeclareMathAccent{\wideparen}{0}{mathx}{"75}


==> tex-common/proof-helpers.tex <==
\RequirePackage{adjustbox}

% http://tex.stackexchange.com/questions/44933
\newcounter{myequation}
\makeatletter
\@addtoreset{equation}{myequation}
\makeatother

% http://tex.stackexchange.com/questions/82535
\newenvironment{proofalign}{\par\nobreak\small\noindent\flalign}{\endflalign}

\newcommand*{\proseDescription}{\paragraph{Prose description.}}
\newcommand*{\paragraphCase}[1]{\paragraph{\uline{#1}}}

\newcommand*{\absurd}[1]{\Absurd{\uline{#1}}}
\newcommand*{\Absurd}[1]{\textcolor{red}{#1}}
\newcommand*{\contradiction}{\Absurd{\bot}}
\newcommand*{\qedLocal}{\text{\ding{234}}\;}

\setlength{\ULdepth}{0.25em}
\newcommand*{\interCaseZero}[1]{%
& \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interCaseOne}[1]{%
& \indent \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interCaseTwo}[1]{%
& \indent\indent \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseZero}[1]{%
& \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseOne}[1]{%
& \indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseTwo}[1]{%
& \indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseThree}[1]{%
& \indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseFour}[1]{%
& \indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseFive}[1]{%
& \indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseSix}[1]{%
& \indent\indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseSeven}[1]{%
& \indent\indent\indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}

\newcommand*{\introCaseDerivationZero}[2]{%
& \textbf{\emph{Case}}\ %
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}

\newcommand*{\introCaseZero}[1]{%
& \textbf{\emph{Case}}\ \uline{#1}.\;%
}

\newcommand*{\introSubcaseZero}[1]{%
& \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseOne}[1]{%
& \indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseTwo}[1]{%
& \indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseThree}[1]{%
& \indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseFour}[1]{%
& \indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseFive}[1]{%
& \indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}

% define \derivationWidth as a proportion of textwidth

\newcommand*{\caseDerivation}[2]{%
\textbf{\emph{Case}}\ %
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}
\newcommand*{\derivation}[2]{%
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}


==> tex-common/relational-composition.tex <==
% Relational composition.
\DeclareSymbolFont{bbsymbol}{U}{bbold}{m}{n}
\DeclareMathSymbol{\bbsemi}{\mathbin}{bbsymbol}{"3B}


==> tex-common/secbreak.tex <==
\RequirePackage{fdsymbol}

\newcommand*{\secbreakchar}{\smblklozenge}
\newcommand*{\secbreak}{
\begin{center}%
   $\secbreakchar\;\secbreakchar\;\secbreakchar$%
\end{center}%
}


==> tex-common/theorem-envs.tex <==
% Not needed for llncs.sty or acmart.cls.
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{definition}{Definition}[subsection]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

% http://tex.stackexchange.com/questions/43966
\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
}
\makeatother


==> tex-common/tilde.tex <==
% https://tex.stackexchange.com/questions/9363/how-does-one-insert-a-backslash-or-a-tilde-into-latex
\newcommand*{\Tilde}{\raise.17ex\hbox{$\scriptstyle\sim$}}


==> tex-common/wavey.tex <==
% http://tex.stackexchange.com/questions/80378. This looks great, but unfortunately doesn't
% work properly with the Listings package; need to come up with an MWE and post a question.
\usepackage{xparse}
\usepackage{marginnote}
\usepackage{soul}
\usepackage{lipsum}
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\newlength\LineWidth
\newlength\Amplitude
\newlength\SegLength

\setlength\LineWidth{0.4pt}
\setlength\Amplitude{1pt}
\setlength\SegLength{5pt}

\definecolor{HLcolor}{RGB}{240,0,0}

% The following code contains a variation of the great code by Antal S-Z
% in his answer to http://tex.stackexchange.com/a/6029/3954
%in TeX.SX

\newcommand\tikzmark[1]{%
  \tikz[overlay,remember picture] \node (#1) {};}

\makeatletter
\newcommand{\highlight@DoHighlight}{
  \draw[HLcolor,line width=\LineWidth,decorate,decoration={zigzag,amplitude=\Amplitude,segment length=\SegLength}]  ($(begin highlight)+(0,-2pt)$) -- ($(end highlight)+(0,-2pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}
\makeatother

\DeclareDocumentCommand\Wavey{O{red}O{1pt}O{5pt}m}{%
  \colorlet{HLcolor}{#1}
  \setlength\Amplitude{#2}%
  \setlength\SegLength{#3}%
  \tikzmark{endquote}\tikzmark{beginquote}\highlight{#4}%
}


==> tex-common/xspace-emdash-fix.tex <==
% https://tex.stackexchange.com/questions/263271
\xspaceremoveexception{-}
\makeatletter
\renewcommand*\@xspace@hook{%
\ifx\@let@token-%
\expandafter\@xspace@dash@i
\fi
}
\def\@xspace@dash@i-{\futurelet\@let@token\@xspace@dash@ii}
\def\@xspace@dash@ii{%
\ifx\@let@token-%
\else
\unskip
\fi
-%
}
\makeatother

